FliT: A Library for Simple and Efficient Persistent Algorithms

Non-volatile random access memory (NVRAM) offers byte-addressable persistence at speeds comparable to DRAM. However, with caches remaining volatile, automatic cache evictions can reorder updates to memory, potentially leaving persistent memory in an inconsistent state upon a system crash. Flush and fence instructions can be used to force ordering among updates, but are expensive. This has motivated significant work studying how to write correct and efficient persistent programs for NVRAM. In this paper, we present FliT, a C++ library that facilitates writing efficient persistent code. Using the library's default mode makes any linearizable data structure durable with minimal changes to the code. FliT avoids many redundant flush instructions by using a novel algorithm to track dirty cache lines. The FliT library also allows for extra optimizations, but achieves good performance even in its default setting. To describe the FliT library's capabilities and guarantees, we define a persistent programming interface, called the P-V Interface, which FliT implements. The P-V Interface captures the expected behavior of code in which some instructions' effects are persisted and some are not. We show that the interface captures the desired semantics of many practical algorithms in the literature. We apply the FliT library to four different persistent data structures, and show that across several workloads, persistence implementations, and data structure sizes, the FliT library always improves operation throughput, by at least $2.1\times$ over a naive implementation in all but one workload.

==> proof-automatic.tex <==

\section{Durable Linearizability of Automatic Transformation}

We first add some detail to the model, to be able to discuss histories more formally.

\subsection{Model Details}
We consider programs that execute data  structure \emph{operations}. Each operation is implemented as a sequence of instructions. An operation is \emph{invoked} when its first instruction is executed, and its \emph{response} occurs immediately after its last instruction is executed. 
%An invocation of an operation $op$ by process $p$ with arguments $args$ is denoted $inv(op, p, args)$, and a response to this operation with return value $r$ is denoted $resp(op, p, r)$. 
An operation's \emph{implementation} specifies a sequence of instructions for processes to execute. \emph{Crash events} can also occur. A crash event erases all values in \dram, but leaves the \pmem{} intact.
A \emph{low-level history} is a sequence of instructions and crash events. A \emph{high-level history} is a sequence of invocations and responses of operations, as well as crash events. Each low-level history maps to some high-level history, and each high-level history can map to a set of low-level histories, representing the different interleavings of instructions that could occur. For an invocation $inv$ in a high-level history $H$, a \emph{matching response} is the next response in $H$ after $inv$ that pertains to the same operation and process. A high-level history is \emph{sequential} if each invocation is immediately followed by a matching response. For each high-level history $H$, and each process $p$, the subsequence of $H$ that includes exactly the invocations and responses that $p$ executed must be sequential.  We say an operation $op$ \emph{happens before} operation $op'$ in $H$, denoted $op <_H op'$, if $op$'s response is before $op'$'s invocation in $H$. This defines a partial order $<_H$ between operations in each high-level history.
%

A data structure $D$ defines a set of operations, along with a \emph{sequential specification}, which defines how the operations behave in a sequential history. 
We consider two histories \emph{equivalent} if (1) they are histories of the same data structure and contain the same set of operations, (2) the return values and the order of invocations and responses of all operations are the same, and (3) the state of \pmem{} after the two histories are the same. 
%\Naama{got rid of legal. Need to rephrase the proof to not use legal.}
A high-level history $H$ with operations of data structure $D$ is \emph{linearizable} if it contains no crash events, and there exists a sequential history $S$ such that (1) $H$ and $S$ are equivalent, (2) $<_H \subseteq <_S$, and (3) $S$ satisfies the sequential specification of $D$. A history is \emph{durably  linearizable}~\cite{izraelevitz2016linearizability} if it is linearizable after all crash events are removed from it.

\subsection{Proof}

\begin{theorem}\label{thm:iz-semantics}
Given a linearizable data structure, if we make all its loads and stores persisted (Definition \ref{def:spec}), then the resulting data structure is durably linearizable.
\end{theorem}

%To prove this theorem, we rely on a useful definition for arguing about different concurrent executions of a data structure.
%
%\begin{definition}
%Two histories are considered \emph{equivalent} if (1) they are legal executions of the same data structure and contain the same set of operations, (2) the return values and the order of invocations and responses of all operations are the same, and (3) the state of memory after the two histories are the same.
%\end{definition}

We begin the proof with the  following lemma, which will help us prove the theorem constructively.

\begin{lemma}\label{lem:iz-semantics}
Consider a linearizable data structure $D$,  and let $D_p$ be an implementation of $D$ in which all loads and stores are \flushed{}. Given a history $H$ of $D_p$ with a single crash at the end, we can construct an equivalent history with no crashes.
\end{lemma}

\begin{proof}
	Consider the set of \flushedm{s} in $H$ that are linearized but not persisted. Let $s$ be the last such store, $p$ be the process that executed $s$, and $m$ be the memory location on which $s$ was executed. For convenience, we say that a  load $\ell$ \emph{sees} a store $s$ if $\ell$ returns the value that $s$ wrote, assuming (without loss of generality) that all values written on memory are unique. 
	We construct an equivalent history $H'$ in which $s$, and all the loads that see $s$, never happen. 
	
	First, note that after $p$ executes $s$, $p$ cannot perform any more stores or complete an operation because otherwise, $s$ would have been persisted by the \interface, by Conditions 3 and 4. Therefore $p$ only performs load instructions after $s$ and removing these loads leads to an equivalent history. 
	
	Suppose some process $p'$ performs a \flushedl{} that sees $s$. After this load, $p'$ cannot perform a store or complete an operation, by the same argument as above. Therefore, removing this load and all later instructions by $p'$ results in an equivalent history. There cannot be any linearized stores to $m$ after $s$ because $s$ was chosen to be the last store that was linearized but not persisted.
	
	Now we have an equivalent history in which $p$ performs no steps after $s$, and no process sees or overwrites the value written by $s$. Since $s$ will be lost after the crash, we can remove $s$ without violating the legality of the history and without affecting the final memory state. 
	
	Applying this argument for each linearized but not persisted store yields an equivalent history in which all visible stores are persisted. Therefore we can remove the final crash event without changing the final memory state. The resulting history is equivalent to $H$ and has no crash events, as desired.
\end{proof}

We are now ready to prove the main theorem.

\begin{proof}[Proof of Theorem~\ref{thm:iz-semantics}]
	Applying Lemma~\ref{lem:iz-semantics} inductively, we can show that a history of the transformed data structure with any number of crash events is equivalent to some history with no crashes. We know that histories with no crashes are linearizable since the original data structure is linearizable, so the transformed data structure is durably linearizable.
\end{proof}

%\begin{proof}
%%Definition: Two histories are considered equivalent if (1) they are legal executions of the same data structure and contain the same set of operations, (2) the return values and the order of invocations and responses of all operations are the same, and (3) the state of memory after the two histories are the same.
%	
%Claim: Consider a linearizable data structure $D$,  and let $D_p$ be an implementation of $D$ in which all loads and stores are \flushed{}. Given a history $H$ of $D_p$ with a single crash at the end, we can construct an equivalent history with no crashes.
%
%\Hao{A persisted store's value only needs to be in transit before the completion of the store.}
%\Hao{Definition 1 needs to talk about operation completions.}
%
%Claim proof: Consider the set of \flushedm{s} in $H$ that are visible but not persisted. Let $s$ be the last such store, $p$ be the process that executed $s$, and $m$ be the memory location on which $s$ was executed. For convenience, we say that a  load $\ell$ \emph{sees} a store $s$ if $\ell$ returns the value that $s$ wrote, assuming (without loss of generality) that all values written on memory are unique. 
%We construct an equivalent history $H'$ in which $s$, and all the loads that see $s$, never happen. 
%
%First, note that after $p$ executes $s$, $p$ cannot perform any more stores or complete an operation because otherwise, $s$ would have been persisted by Definition~\ref{def:spec}. Therefore $p$ only performs load instructions after $s$ and removing these loads leads to an equivalent history. 
%
%Suppose some process $p'$ performs a \flishedl{} that sees $s$. After this load, $p'$ cannot perform a store or complete an operation, by the same argument as above. Therefore, removing this load and all later instructions by $p'$ results in an equivalent history. There cannot be any stores to $m$ after $s$ because $s$ was chosen to be the last store that was visible but not persisted.
%
%Now we have an equivalent history in which $p$ performs no steps after $s$, and no process sees or overwrites the value written by $s$. Since $s$ will be lost after the crash, we can remove $s$ without violating the legality of the history and without affecting the final memory state. 
%
%Applying this argument for each visible but not persisted store yields an equivalent history in which all visible stores are persisted. Therefore we can remove the final crash event without changing the final memory state. The resulting history is equivalent to $H$ and has no crash events, as desired.
%
%Applying the claim inductively, we can show that a history of the transformed data structure with any number of crash events is equivalent to a history with no crashes. We know that histories with no crashes are linearizable since the original data structure is linearizable, so the transformed data structure is durably linearizable.
%\end{proof}
